The Physics and Nuclear Nonproliferation Goals of WATCHMAN: A WAter CHerenkov Monitor for ANtineutrinos

This article describes the physics and nonproliferation goals of WATCHMAN, the WAter Cherenkov Monitor for ANtineutrinos. The baseline WATCHMAN design is a kiloton scale gadolinium-doped (Gd) light water Cherenkov detector, placed 13 kilometers from a civil nuclear reactor in the United States. In its first deployment phase, WATCHMAN will be used to remotely detect a change in the operational status of the reactor, providing a first- ever demonstration of the potential of large Gd-doped water detectors for remote reactor monitoring for future international nuclear nonproliferation applications. During its first phase, the detector will provide a critical large-scale test of the ability to tag neutrons and thus distinguish low energy electron neutrinos and antineutrinos. This would make WATCHMAN the only detector capable of providing both direction and flavor identification of supernova neutrinos. It would also be the third largest supernova detector, and the largest underground in the western hemisphere. In a follow-on phase incorporating the IsoDAR neutrino beam, the detector would have world-class sensitivity to sterile neutrino signatures and to non-standard electroweak interactions (NSI). WATCHMAN will also be a major, U.S. based integration platform for a host of technologies relevant for the Long-Baseline Neutrino Facility (LBNF) and other future large detectors. This white paper describes the WATCHMAN conceptual design,and presents the results of detailed simulations of sensitivity for the project's nonproliferation and physics goals. It also describes the advanced technologies to be used in WATCHMAN, including high quantum efficiency photomultipliers, Water-Based Liquid Scintillator (WbLS), picosecond light sensors such as the Large Area Picosecond Photo Detector (LAPPD), and advanced pattern recognition and particle identification methods.

==> mh.tex <==
\subsection{Study of Mass Hierarchy Sensitivity at the WATCHMAN Site} 
\label{sec:mh}

It has been known for some time that a reactor experiment with a large, ultra-high resolution detector at a distance
of roughly 50 km could potentially determine the neutrino mass ordering. There have been no detailed studies of what
a smaller detector at a closer distance might do. While the effect on the neutrino spectrum decreases as the distance
decreases, this is offset somewhat by the $1/r^2$ increase in neutrino interaction rate.

We have performed preliminary studies into the possibility of performing a neutron mass ordering experiment at the WATCHMAN site
following the completion of Phases 1 and 2. This experiment would require the use of a high light yield Liquid Scintillator (LS)
rather than Gd-H2O or WbLS. A detector larger than 1 kiloton would also likely be required. WATCHMAN
will make use of a method for determining the mass order that follows from the observation of Sergei Petcov (and others), \cite{PetcovNN}
 which states that the electron antineutrino survival probability can be written in a form that contains four terms, as shown in Equation.~\ref{eq:RxDisappearance}
 It has been recognized by members of the WATCHMAN collaboration that it is possible to use Fourier transforms to pick
 out the hierarchy dependent terms in this equation:

\begin{equation}
\begin{aligned}
P_{ee} =&1 - \cos^4(\theta_{13})\sin ^2(2\theta_{12})\sin^2(\Delta_{21})
        &+ \cos^2(\theta_{12})\sin^2(2\theta_{13})\sin^2(\Delta_{31})
        &+ \sin^2(\theta_{12})\sin^2(2\theta_{13})\sin^2(\Delta_{32})
\end{aligned}
\label{eq:RxDisappearance}
\end{equation}


In equation~\ref{eq:RxDisappearance}, $\theta_{12}$ and $\theta_{13}$ are mixing angles, $\Delta_{ji}=1.27(|\delta m2_{ji}|L)/E_{\nu}$ controls
 the oscillations, with  $\delta m2_{ji}=m_{j}^2-m_{i}^2$ as the neutrino mass-squared difference of $\nu_j$ and $\nu_i$ in $eV^2$, $L$ is the
 neutrino flight distance in meters, and $E_{\nu}$ is the neutrino energy in MeV.  Three oscillating terms, each  with a ``frequency'' in L/E
 space specified by $\delta m2_{ji}$, suppress the survival probability.  The amount of suppression provided by each term relative to that of
 the second term is $\sin^2(2\theta _{12})/\tan^2(\theta_13) : 1 : \tan^2(\theta_{12})$.  The first term with the lowest  ``frequency''
 dominates.  It is responsible for the deficit of solar neutrinos and the conspicuous spectral distortion of reactor antineutrinos [2].
   Sensitivity to these oscillations is greatest when $\Delta_{21}=\pi/2$, which provides maximum suppression by the dominant term and
 thereby the highest  signal-to-noise ratio.  For the normal hierarchy of neutrino masses $(m3>m2>m1)$, $\Delta_{31}$ is slightly greater
 than $\Delta_{32}$, giving the second term a slightly higher ``frequency'' than the third term.  Whereas for the inverted hierarchy of
 neutrino masses $(m2>m1>m3)$, $\Delta_{31}$ is slightly smaller than $\Delta_{32}$, giving the second term a slightly lower ``frequency''
 than the third term.  It is thus possible to determine neutrino mass hierarchy by  resolving the small ($\sim 3\%$) difference in
 the ``frequency'' of the second and third terms.

%\begin{figure}
%\begin{center}
%\includegraphics[width=0.45\textwidth]{53kmLEnosmear.png}
%\includegraphics[width=0.45\textwidth]{53kmLEsmear35.png}
%\caption{Inverse beta decay event rate versus neutrino energy for a detector 55 km from a nuclear reactor,
% showing unoscillated and oscillated 
%spectrum for both normal and inverted neutrino mass ordering. No resolution smearing (left) and with $3.5\%/\sqrt{E}$
% smearing (right).}
% \label{fig:53km}
%\end{center}
%\end{figure}

%This is best illustrated at a long distance. Figure~\ref{fig:53km} shows the unoscillated antineutrino $L/E$ distribution
%for $L=53~km$ and the oscillated spectrum for both normal and inverted ordering. The small oscillations are due to the $\theta_{13}$
% terms in equation~\ref{eq:RxDisappearance}. At this distance, many oscillations are observed and can be Fourier analyzed to determine the
% hierarchy. The number of cycles is, however, effectively reduced by detector energy smearing, as shown in the right hand side of
% Figure~\ref{fig:53km}. Here, an energy resolution described by $\sigma_E = 3.5\%/\sqrt{E(1\; MeV}$ is used, 
%which is better by a factor of two than other detectors---such as KamLAND---but, in principle, achievable.


%The rapid oscillations in Figure~\ref{fig:53km}, consist of the last two terms of Equation~\ref{eq:RxDisappearance},
% and one cannot easily distinguish the two hierarchy cases visually. More importantly, the uncertainty in $\Delta_{32}^2$
% means that the whole spectrum can be shifted left or right on the order of one oscillation. Hence it is the frequency
% rather than the phase that is important for the measurement. By performing a Fourier Transform (FT) in $L/E$ space, it is
% possible to discriminate between the mass
%hierarchies. The transform in the neighborhood of $\Delta_{32}^2$ term is show in Figure~\ref{fig:FT}.
% It can be seen that the left and right peaks are not equal in amplitude since one depends upon $\sin^2(\theta_{12})$ and the
% other on $\cos^2(\theta_{12})$, hence the two possible hierarchies can be distinguished by the shape of the power spectrum.

%\begin{figure}
%\begin{center}
%\includegraphics[width=0.45\textwidth]{53kmFTnosmear.png}
%\includegraphics[width=0.45\textwidth]{53kmFTsmear35.png}
%\caption{The FT power spectrum of inverted and mass hierarchy $L/E$ distributions at 53km. 
%No resolution smearing (Left) and with $3.5\%/\sqrt{E}$ smearing (right).}
%\label{fig:FT}
%\end{center}
%\end{figure}
 


\begin{figure}
\begin{center}
\includegraphics[width=0.45\textwidth]{13kmLEsmear35.png}
\includegraphics[width=0.45\textwidth]{13kmFTsmear35.png}
\caption{(Left) the $L/E$ distribution (with $3.5\%/\sqrt{E}$ smearing) for the WATCHMAN 13 km baseline.
  (Right) The FT power spectrum for this case. An exposure of 188 $GW\cdot kton\cdot years$ is assumed.}
\label{fig:WATCHMANMH}
\end{center}
\end{figure}
 



To assess the potential sensitivity, we have performed a preliminary likelihood analysis as follows:\

\begin{enumerate}
\item Make a trial likelihood FT power function ($f_{i}(\Delta)_{NH,IH}$)
for both normal and inverted hierarchy by randomly selecting oscillation parameters
from the experimental measurements, assuming uncertainties are Gaussian. Some parameters have experimental central values and
uncertainties that depend on the hierarchy: these parameters were taken into account in the analysis.
\item Make a template ($F(\Delta)=(1/N) \Sigma f_{i}(\Delta)$) for each hierarchy by averaging over 10,000 trials
\item Make a weighting template ($W(\Delta) = (1/N)\Sigma|F(\Delta)-f_{i}(\Delta)|$) for each 
hierarchy based on the average deviation of individual trails with the template
\item Assuming the central measured values of the oscillation parameters, make 1000 fake experiments, each with a power
 spectrum $g(\Delta)$ and for each calculate the likelihood  
($L$) of being normal or inverted hierarchy via $L = \Sigma |F(\Delta)-g(\Delta)|/W(\Delta)$
\end{enumerate}

The results of this test are shown in Figure~\ref{MHL}, assuming a 5 kiloton fiducial volume. Since there is clearly a reasonable potential for sensitivity,
 we have continued to study this possibility for the Fairport site. A future study will account for detector effects using the WATCHMAN simulation package. 
 
 We conclude that the existing WATCHMAN detector fiducial volume would be too small - a detector of at least 5 kilotons would be required, plus a liquid scintillator (or possibly WbLS at high concentration) fill. Studies of other sites (for example Boulby, which has a 25 km baseline) are also being investigated.

\begin{figure}
\begin{center}
\includegraphics[width=0.8\textwidth]{MH_Likelihood1.png}
\caption{Separation of inverted and normal mass hierarchies via FT-based likelihood analysis at the WATCHMAN site.}
\label{MHL}
\end{center}
\end{figure}




==> reactorDir.tex <==

\subsection{Reactor Antineutrino Directionality}

\label{sec:reactorDir}

xxx - Caveat: There is an issue concerning the bonsai reconstruction software that causes a small fraction of PMT gamma ray backgrounds to reconstruct in a random location within the fiducal volume, even when the fit seems to have converged on a good vertex location (according to bonsai).  The effect is that the distance between a reconstructed vertex and the "truth" vertex doesn't follow a regular statistical distribution with vanishing tails - but that (for a small fraction of events) the tails don't vanish at any distance. If, in the next few weeks we can figure out this problem and identify/remove these badly reconstructed events, then it may indeed be possible, as shown below, to successfully identify the source direction of an antineutrino flux via antineutrino elastic scattering. For now this section does not include a proper treatment of PMT backgrounds.  We have instead focussed on finding out if reactor directionality is doable given all the other backgrounds that we expect, including the higher levels of radionuclide backgrounds at WATCHMAN relative to Super-K.  Please note, the problem here may not have anything to do with bonsai itself, but may be due to the way we have implemented it, or a tuning issue. Stay tuned  - Steven Dazeley. - xxx
\\
\\
\\
\\
The inverse beta decay (IBD) reaction on free protons allows, via a measurement of the resulting positron energy, a good determination of the antineutrino energy (\cite{An:2012eh}, \cite{dayabay:2013}, \cite{reno:2012}).  However, the direction of the antineutrino is poorly correlated with either the direction of the positron, or its location with respect to the neutron capture, making a determination of the direction of the antineutrino difficult. Here we investigate the potential of using the elastic scattering reaction \mbox{( $ \bar {\nu} + e^{-} \rightarrow   \bar {\nu} + e^{-} $ )}, in WATCHMAN, to statistically determine the direction of an incoming antineutrino flux. 

The standard model total elastic scattering cross section, including both the charged and neutron current components, can be written as follows:

\begin{equation}  
\label{totalCrossSection}
\sigma (E_{\nu}) = \left(\frac{G_{F}^{2} m_{e} E_{\nu}}{2\pi}\right) \left( \frac{1}{3} (1 + 2sin^{2}(\theta_{W})^{2} + 4sin^{4}(\theta_{W}) \right) \approx (7.8 \times 10^{-45}) m_{e} E_{\nu}  \frac{cm^{2}}{MeV^{2}}
\end{equation}

Where $\theta_{W}$ is the Weinberg angle and $sin^{2}(\theta_{W}) \approx 0.23$.  Figure~\ref{fig:crossSecFigure} compares this cross section with the more commonly used IBD cross section as a function of antineutrino energy. While it is certainly true that the elastic scattering cross section is comparatively small, we note that the difference between the two decreases with decreasing energy, and the number of electron scattering targets is 5 times the number of IBD free proton targets in water. 

The electron scattering angle, $\theta$, is the angular difference between the antineutrino direction and the electron direction. Scattered electron energies range from a maximum value just shy of the incoming antineutrino energy at $\theta = 0$ down to zero. The maximum energy is

\begin{equation}  
\label{scatteringAngle}
T_{e}^{max} = \frac{2E_{\nu}^{2}}{m_{e} + 2E_{\nu}}
\end{equation}

An elastic scattering generator has been developed for the GEANT4 simulation of the WATCHMAN detector. It was motivated by a desire to determine the sensitivity of a potential IsoDAR deployment at WATCHMAN to non-standard electron scattering interactions (see section~\ref{sec:NSI}). The generator was then adapted for reactor antineutrinos, using an analytical expression for the antineutrino flux \cite{VogelEngel} as a function of energy. More recent determinations of the spectrum (such as from \cite{PhysRevC.84.024617}, or \cite{PhysRevC.83.054615}), only extend down to 2 MeV, relevant to IBD calculations.  We compared the predicted interaction rates of both models in WATCHMAN above 2 MeV to check for consistency, and found them to be consistent to within $\sim 10\%$.

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.45\textwidth]{scatteringCrossSection.png}
\caption{The interaction cross section for inverse beta decay (IBD) on a proton, and elastic scattering on an electron, as a function of antineutrino energy.}
\label{fig:crossSecFigure}
\end{center}
\end{figure}

The generator calculates the number of interactions based on the flux and energy distribution of the incoming antineutrinos, then generates a sample of electron scatter events, sampling position, energy and direction, within the fiducial volume. It calculates the incoming antineutrino flux for any desired reactor uranium or plutonium isotopic content. The isotopic fission fractions used here were $^{235}U (0.5)$, $^{238}U (0.09)$, $^{239}Pu (0.35)$, $^{240}Pu (0.06)$, consistent with a light water reactor of the Perry type in mid fuel cycle.  The generated scattered electron sample was then simulated in the WATCHMAN detector simulation, which includes detector physics effects such as Cherenkov photon generation, photon transport, reflections, PMT efficiency, electronic charge/timing resolution and so on. The size of the inner detector volume was increased as much as possible given the constraints of the detector location and overall size, to a radius of 6.9 meters, in anticipation of the need for extra fiducial volume. The events were then reconstructed using the "bonsai" vertex fitter, adapted from Super-K \cite{Watchman:BONSAI}. Figure~\ref{fig:scatterE} shows the distribution of an arbitrary number of scattered electron energies in WATCHMAN from a nearby reactor, together with the fraction that successfully trigger the detector.  The detector trigger efficiency reaches $100\%$ at approximately 1.6 MeV. Note the heavy concentration of low energy scattered electrons that fail to trigger.  

\begin{table}[htbp]
\caption{The reactor elastic scattering like background events expected after 5 years running time at WATCHMAN over an energy range extending up to 15 MeV, assuming the full 1 Kton fiducial volume.}
    \begin{tabular}{|c|c|}
\hline
    \textbf{Event Type}  &  \textbf{Background (5 years)}  \\
    \hline
    Misidentified IBD & 3650 \\
    $^{208}Tl$ gamma rays  & 1154  \\
    Steel Support Gamma rays & 437 \\
    Rock Gamma rays & 1025 \\
    $^{8}B$ Solar Neutrinos &  2180 \\
    Radionuclide $^{8}B$ &  4880  \\
    Radionuclide $^{8}Li$ &  12720 \\
    Radionuclide $^{11}Be$ &  3690  \\
    Radionuclide $^{15}C$ & 2320 \\
    Radionuclide $^{16}N$ & 75750  \\
    \textbf{Total Backgrounds} & \textbf{107800} \\


\hline
 \end{tabular}
  \label{tab:DirBackgroundEvents}
\end{table}


\begin{figure}
\begin{center}
\includegraphics[width=0.45\textwidth]{ReactorTriggerEnergy.eps}
\caption{The distribution of scattered electron energies due to elastic scattering in WATCHMAN from a nearby reactor.  Note the trigger efficiency reached $100\%$ efficiency at approximately 1.6 MeV.  The trigger condition is 16 PMT hits within 200 nanoseconds (left). The subset of electron scatters that trigger WATCHMAN in one year compared with the predicted level (and energy distribution) of all the backgrounds (right).}
\label{fig:scatterE}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=0.32\textwidth]{reactor_backgrounds_E.eps}
\includegraphics[width=0.32\textwidth]{reactor_backgrounds_PE.eps}
\includegraphics[width=0.32\textwidth]{reactor_signalBackground_PE.eps}
\caption{The energy distributions of the reactor antineutrino elastic scattering background components (left). The WATCHMAN detector response as a function of detected photoelectrons, according to the GEANT4 WATCHMAN simulation (middle). To the right the subset of electron scatters that trigger WATCHMAN in one year compared with the predicted level (and energy distribution) of all the backgrounds.}
\label{fig:reactorBackgrounds}
\end{center}
\end{figure}

The apparent directional sensitivity of WATCHMAN will depend upon the amount of non-directional background present. Some of the estimates presented in Table~\ref{tab:DirBackgroundEvents}, including gamma rays from the wall and solar neutrinos were scaled from IsoDAR/KamLAND estimates \cite{Conrad:2013sqa}, adjusting for the larger fiducial volume of WATCHMAN. We have not yet included estimates of PMT or radon related backgrounds. The PMT background estimates await the completion/tuning of a vertex fitter, while the radon levels will depend heavily on the technology used to recycle and clean the water. Our interest here is simply to study the feasibility of directionality, assuming the detector and water system designs will render the detector component/water radioactivity backgrounds subdominant. The Misidentified IBD background from the Perry reactor was estimated assuming that WATCHMAN would detect 10 IBD events per day from the Perry reactor, with a neutron detection inefficiency of $20\%$ - leading to 2 backgrounds per day. The largest irreducible background component is due to cosmogenic radionuclides. While these have never been measured in water, the yields of a selection of candidate radionuclides have recently been estimated for the Super-Kamiokande detector \cite{LiBeacom2014}, using a FLUKA simulation. To scale to the depth of WATCHMAN, we assumed the production mechanism is primarily associated with showering (high energy) muons passing through the detector. A GEANT4 simulation of muon flux as a function of depth and energy \cite{ReynaMuons}, and a representative sea level muon energy spectrum was used to predict the rate of showering muons at WATCHMAN, relative to KamLAND, and found to be 2.6 times higher. At this rate, in order to maintain an equivalent live time to KamLAND, we reduced the 5 second veto to 2 seconds following each showering muon. 

\begin{table}[htbp]
\caption{The most dangerous (for the NSI experiment) long lived cosmogenic radionuclide backgrounds for a water-based target. The predictions (taken from \protect\cite{LiBeacom2014}) were generated from a FLUKA study. We include here only those nuclei that produce a high yield of beta/gamma decays with a lifetime longer than $\sim 1$ second.  The radionuclide isotopes of interest to the organic scintillator experiment include only a subset of these, $^{11}$Be, $^{8}$Li and $^{8}$B \protect\cite{Conrad:2013sqa}.}
\begin{tabular}{|c|c|c|c|c|}
\hline
    \textbf{Isotope}  &  \textbf{Half-life (s)} & \textbf{Decay Mode} & \textbf{Yield} $\bf{(\times 10^{-7} \mu^{-1} g^{-1} cm^{2} )}$   &    \textbf{Primary Process} \\
    \hline
    $^{16}N$ & $7.13$ & $\beta^{-} \gamma (66\%),  \beta^{-} (28\%)$ & $18$ & (n,p) \\
    $^{15}C$ & $2.449$ &  $\beta^{-} \gamma (63\%),  \beta^{-} (37\%)$ & $0.8$ & (n,2p) \\
    $^{11}Be$ & $13.8$ & $\beta^{-} (55\%),   \beta^{-} \gamma (31\%)$ & $0.8$ &  (n,$\alpha +$ 2p) \\
    $^{8}B$ & $0.77$ & $\beta^{+}$ & $5.8$ &         ($\pi^{+},\alpha + $ 2p $+$ 2n) \\
    $^{8}Li$ & $0.84$ &  $\beta^{-}$ & $13$ & ($\pi^{-},\alpha + ^{2}H$ $+$ p $+$ n) \\    
    
        \hline
 \end{tabular}
  \label{tab:LiBeacomRadNucs}
\end{table}    

The yields of each radionuclide are converted to rates at the KamLAND/Super-Kamiokande depth using:
\begin{equation}  
 \label{nsi}
R_{i} = \rho Y_{i} L_{\mu} R_{\mu} 
 \end{equation}
Where $Y_{i}$ is the yield of the i'th isotope, $L_{\mu}$ is the average distance that muons travel through the detector volume, $\rho$ is the density of the target and $R_{\mu}$ is the muon rate. We use KamLAND as our baseline detector since the mean muon path length is known ($874cm$ inside the $1150 m^{3}$ balloon), the volume is similar to WATCHMAN \cite{KamLANDMuons}, and the depth is the same as Super-Kamiokande.  We then calculate the expected radionuclide rates in a hypothetical WATCHMAN sized detector at the same depth as KamLAND, then scale to the true WATCHMAN depth, assuming as before the showering muon rate is 2.6 times higher.  Finally, we account for the livetime following the muon veto ($82\%$).

\begin{figure}[h]
\begin{center}
\includegraphics[height=0.3\textwidth]{cosineScatter.eps}
\includegraphics[height=0.3\textwidth]{cosineScatterPlusBack.eps}
\caption{the angle between the incoming antineutrino direction and the reconstructed recoil electron direction ($cos \theta $) for a one year data run at WATCHMAN (left). A value of +1 implies the electron direction equals that of the antineutrino. To the right is a similar one year simulation of WATCHMAN events, including the anticipated background. Background events are assumed to have a flat $cos \theta $ distribution.}
\label{fig:cosineDist}
\end{center}
\end{figure}

Figure~\ref{fig:reactorBackgrounds} shows the energy distribution of the various background components considered here and the corresponding WATCHMAN detector response in terms of detected photoelectrons over a timeframe of 1 year. The radionuclide component peaks at approximately 100 photoelectrons. The largest individual radionuclide component is $^{16}N$ (see Table~\ref{tab:LiBeacomRadNucs} and Table~\ref{tab:DirBackgroundEvents}).  Figure~\ref{fig:reactorBackgrounds} shows a comparison of the reactor scattering and the total background detector response distributions. We note that the reactor elastic scattering signal rises at low energies, while the total background level is falling.  If the background at WATCHMAN is indeed dominated by radionuclides, which peak at $\sim 7 MeV$ or $\sim 100$ photoelectrons, it may be possible to significantly reduce them by imposing an upper energy cut, perhaps near $\sim 65$ photoelectrons.  In this case, for illustrative purposes, we applied an upper energy cut at 65 photoelectrons.  Figure~\ref{fig:cosineDist} shows the plot of the cosine scattering angle distribution for a one year data run. We assume the background is isotropic, producing a flat cosine distribution.

Figure~\ref{fig:cosineDist} shows the reconstructed distribution of scattering angles (in $cos \theta $) using the bonsai fitter (+1 corresponds to a scattering angle $\theta = 0$).  Background is assumed to have an isotropic distribution of directions, adding a flat component to the cosine distribution. When running the elastic scattering simulation over many thousands of events, we found that the $cos \theta $ distribution takes on the shape of an exponential curve, peaking at $cos \theta = +1$.  In Figure~\ref{fig:reactorBackgrounds} we use the normalization uncertainty of the exponential fit to obtain the uncertainty associated of our expected signal.  An analysis method such as this would be possible at WATCHMAN if a directional calibration source is employed, such as the electron accelerator at Super-Kamiokande. This would allow a measurement of the slope of the exponential. If a directional source is not available then perhaps an analysis cut on the scattering angle will suffice.  Here we apply both methods and compare. The best $cos \theta$ cut maximizes the statistical significance of the signal at $cos \theta = xxx$. In Figure~\ref{fig:elasticScatterSigmas}, 64 successive independent simulations were run, each of a one year data including signal and background. Fitting an exponential, allowing the normalization to float and fixing the slope, we find the mean statistical significance predicted from each one year data set was $5.5 \sigma$. Alternatively, if we make no assumptions about the shape of the $cos \theta $ distribution, simply applying an independent analysis cut on the scattering angle for each of the 64 year long data runs, the resulting mean statistical significance was $5.1 \sigma $. 

\begin{figure}[h]
\begin{center}
\includegraphics[height=0.3\textwidth]{sigma_sigma_YInterceptMethod.eps}
\caption{A plot of the statistical significance for a succession of 64 independent year long simulated data sets.  The average result is a $5.5 \sigma$ detection over one year. }
\label{fig:elasticScatterSigmas}
\end{center}
\end{figure}

\subsubsection{Detector Radioactive Backgrounds}

We have until now ignored the effects of two classes of background, gamma ray emission from the PMTs and water borne radon.  Table~\ref{tab:PMT_UThK_Table} summarizes the levels of $^{238}U$, $^{232}Th$ and K in the glass of the primary candidate PMTs. The decay chains from these impurities produce a 2.6 MeV gamma ray from $^{208}Tl$, and $1.4 MeV$ from $^{40}K$.  The $^{238}U$ decay chain generally results in the formation of radon which can migrate into the water and result in a $^{214}Bi$ decay. We consider the $2.6 MeV$ and $1.4 MeV$ gamma rays first. In most cases PMT sourced gamma rays interact well outside the fiducial volume. However, the vertex fitter will reconstruct the location of the event with some uncertainty. The black curve in Figure~\ref{fig:PMTGammaBackgrounds} shows the distance from the reconstructed vertex position to the nearest PMT generated from a set of 840,000 simulated PMT gamma rays. Only events that reconstruct inside the PMT cylinder are shown. Given that the nominal kiloton WATCHMAN fiducial volume extends to within 1.5 meters of the PMTs, clearly a significant number of the these background events will be reconstructed inside. In fact two distinct groups of events are revealed.  At small PMT distances a population of events are distributed exponentially as indicated in the figure. At larger distances we have almost a flat distribution, possibly following at least one or two additional exponential components. The situation improves somewhat if the lowest energy events with a poor fit (low log likelihood) are removed, as shown by the blue curve. The vertex fitter we are using, called "bonsai" was adapted from the fitter at Super-Kamiokande.  At the present time the fitter has not been optimally tuned for WATCHMAN. It is possible that better performance will be achieved in the future.  For now we estimate the likely effect of this background on our directionality signal using the current bonsai fitter. 

\begin{table}[htbp]
\caption{U/Th/K glass impurity measurements from four candidate PMTs. Measurements of single PMT samples at the Berkeley low background counting facility.}
\begin{tabular}{|c|c|}
\hline
\textbf{Candidate PMT Type} & \textbf{U/Th/K Impurities} \\
\hline
12-inch Hamamatsu  & $^{232}Th : 1.33 \times 10^{-6} $ g/g \\
 (regular glass) & $^{238}U :  0.34 \times 10^{-6} $ g/g \\
& $K :  260 \times 10^{-6} $ g/g \\
\hline
 12-inch Hamamatsu & $^{232}Th : 0.134 \times 10^{-6} $ g/g \\
  (low background glass) & $^{238}U : 0.043 \times 10^{-6} $ g/g \\
 & $K :  36 \times 10^{-6} $ g/g \\
 \hline
 11-inch ADIT/ETL & $^{232}Th :  0.03 \times 10^{-6} $ g/g \\
  (low background glass) & $^{238}U : 0.03  \times 10^{-6} $ g/g \\
  & $K :  60 \times 10^{-6} $ g/g \\
\hline
10-inch Hamamatsu & $^{232}Th :  0.03 \times 10^{-6} $ g/g \\
 (low background glass, from Double Chooz) & $^{238}U :  0.07 \times 10^{-6} $ g/g \\
 & $K :  20 \times 10^{-6} $ g/g \\
\hline
 \end{tabular}
  \label{tab:PMT_UThK_Table}
\end{table}

\begin{figure}[h]
\begin{center}
\includegraphics[height=0.3\textwidth]{distanceToPMTs_All.eps}
\caption{Detector background events plotted as a function of reconstructed vertex distance from the PMTs. After requiring the number of PMTs hit to be greater than 20, and the log likelihood of the reconstructed vertex to be greater than 20, approximately half of the backgrounds are eliminated.  Additionally, PMT events reconstructed well inside the fiducial volume are significantly reduced.}
\label{fig:PMTGammaBackgrounds}
\end{center}
\end{figure}

As indicated by the blue line in Figure~\ref{fig:PMTGammaBackgrounds}, fitter performance can be improved by removing the lowest energy events ($\leq 20$ PMT hits), with a small log likelihood associated with the fit ($< 20$). The remaining events largely follow a single exponential distribution. However, we note the possibility of an extra, small, and slightly longer exponential component, extending further from the PMTs. Figure~\ref{fig:PMTGammaBackgrounds} shows both fits, however we do not have enough events to determine if the 2nd component is significant. Table~\ref{tab:PMTBackgroundTable} shows the expected rates of background as a function of fiducial volume, assuming the background follows a single, or double exponential shape.

\begin{table}[htbp]
\caption{The expected background event rates at WATCHMAN due to gamma ray emission from the PMTs. A range of fiducial volumes and potential PMT types are considered. The PMT types are represented as follows: "12Reg" - regular glass 12-inch Hamamatsu, "12Low" - low background 12-inch Hamamatsu, "11Low" - low background ETL, "10Low" - low background Hamamatsu. In each of the columns with a range of values, the low number refers to background calculated assuming it follows a single exponential as a function of distance from the PMTs, the high value assumes a small but more gradual exponential (see \protect{Figure~\ref{fig:PMTGammaBackgrounds}}).}
    \begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Buffer Thickness}  &  \textbf{Fiducial Volume} & \multicolumn{4}{ c| }{\textbf{Expected Background Rate}} \\
meters & tonnes & \multicolumn{4}{ c| }{\textbf{(Events per day)}} \\
    \hline
    & & \textbf{12Reg} & \textbf{12Low} & \textbf{11Low} & \textbf{10Low} \\
    \hline
  2.6  & 500 & $3515 \rightarrow 7030$ & $348 \rightarrow 696$ & $75 \rightarrow 149$ & $59 \rightarrow 118$ \\
  2.8  & 430 & $1760 \rightarrow 3830$ & $174 \rightarrow 380$ & $37 \rightarrow 81$ &  $30 \rightarrow 64$ \\
  3.0 & 370 & $800 \rightarrow 2080$ & $79 \rightarrow 206$ & $17 \rightarrow 44$ & $13 \rightarrow 35$ \\
   3.2  & 320 & $415 \rightarrow 1120$ & $41 \rightarrow 111$ & $9 \rightarrow 24$ & $7 \rightarrow 19$ \\
 3.4 & 270 & $192 \rightarrow 575$ & $19 \rightarrow 57$ & $4 \rightarrow 12$ & $3 \rightarrow 10$ \\
  3.6 & 225 & $80 \rightarrow 320$ & $8 \rightarrow 32$ & $1.7 \rightarrow 7$ & $1.3 \rightarrow 5$ \\
  3.8 & 187 & $29 \rightarrow 166$ & $2.8 \rightarrow 16$ & $0.6 \rightarrow 4$ & $0.5 \rightarrow 3$ \\
    \hline
 \end{tabular}
  \label{tab:PMTBackgroundTable}
\end{table}
    

The fact that the reconstructed vertex positions of PMT backgrounds seem to follow an exponential distribution is encouraging news for reactor directionality in general. It implies that PMT backgrounds will be subdominant given sufficient buffer thickness, and a large enough detector. We compile the total backgrounds expected after five years in Table~\ref{tab:detectorBackgrounds}, assuming low background 10-inch PMTs.

Radon calculation is not done yet.  Place here xxx then include in table

\begin{table}[htbp]
\caption{The expected total backgrounds after 5 years run time, including $82\%$ live time.  Included here are PMT gamma ray backgrounds from \protect{Table~\ref{tab:PMTBackgroundTable}} and all the non-PMT backgrounds from \protect{Table~\ref{tab:DirBackgroundEvents}}. Low/High PMT refers to PMT backgrounds either reconstructed according to a single exponential distribution with respect to the PMT distance, or a double exponential distribution respectively (See blue curve of \protect{Figure~\ref{fig:PMTGammaBackgrounds}}).}
\begin{tabular}{|c|c|c|c|c|}
\hline

Fiducial Volume & \multicolumn{2}{ c| }{11Low} & \multicolumn{2}{ c| }{10Low} \\
\hline
 & Low PMT & High PMT & Low PMT & High PMT \\
 \hline
 225 & 3200 & 11130 & 2600 & 8130 \\
 187 & 1555 & 6640 & 1295 & 5140 \\
    \hline
 \end{tabular}
  \label{tab:detectorBackgrounds}
\end{table}



\subsubsection{Conclusions}

The results of this simulation study show that in principle a kiloton sized water Cherenkov WATCHMAN detector may be sensitive to the directional source of a flux of reactor antineutrinos from the Perry reactor under the following conditions: First, statistically, the scenario we have investigated here is a directional search of an incoming antineutrino signal tested with respect to an assumed location.  If no suspected reactor location is known a statistical penalty would need to be paid for testing for multiple directions. We have not investigated that scenario here. Secondly, low energy radioactive backgrounds from the detector walls, PMTs and radon in the water are assumed to be a subdominant background here, relative to cosmogenically sourced radionuclides. This can be achieved with a smaller fiducial volume after 5 years run time only if low background PMTs are used. The vertex fitter performance will also be an extremely important factor, it must not reconstruct too many PMT backgrounds inside the fiducial volume. Stringent cleanliness procedures would need to be put in place to ensure detector components do not contribute further to the background. What these results show is that reactor directionality in WATCHMAN is an extremely difficult experiment. However it seems that the capability is not ruled out on the basis of reasonable assumptions of radionuclide backgrounds, solar neutrinos, or misidentified IBD antineutrinos from the Perry reactor. However successful directional reconstruction will depend in large part on the level of detector cleanliness achieved, PMT radioactivity levels, and on radon levels in the water.
 





